Singular bifurcations in a modified Leslie-Gower model

We study a predator-prey system with a generalist Leslie-Gower predator, a functional Holling type II response, and a weak Allee effect on the prey. The prey's population often grows much faster than its predator, allowing us to introduce a small time scale parameter $\varepsilon$ that relates the growth rates of both species, giving rise to a slow-fast system. Zhu and Liu (2022) show that, in the case of the weak Allee effect, Hopf singular bifurcation, slow-fast canard cycles, relaxation oscillations, etc., exist. Our main contribution lies in the rigorous analysis of a degenerate scenario organized by a (degenerate) transcritical bifurcation. The key tool employed is the blow-up method that desingularizes the degenerate singularity. In addition, we determine the criticality of the singular Hopf bifurcation using recent intrinsic techniques that do not require a local normal form. The theoretical analysis is complemented by a numerical bifurcation analysis, in which we numerically identify and analytically confirm the existence of a nearby Takens-Bogdanov point.

==> sections/secondayequilibria.tex <==
\hjk{maybe move this section later?}

\hjk{Under certain parameter values, a secondary equilibrium point of the slow dynamics appears on ${\mathcal M}_0^{1,r}$, see Theorem \ref{teo1}. This has important consequences for the dynamics, therefore we provide more details on local dynamics of such equilibria. } \hjk{Do we need to show that these equilibria appear only on the repelling part, or is it obvious?}

\hjk{In this section, we study the stability of the positive equilibrium points by focusing on the cases $C=-AMQ$ (Theorem \ref{teo1}, case 2), and $C<-AMQ$ (Theorem \ref{teo1}, case 3). In particular, we first consider the case where, upon variation of $Q$, one passes from $2$(b) to $2$(a) in Theorem \ref{teo1}. After that, we treat the case corresponding to $3$ in Theorem \ref{teo1}.}

\subsection{Case \texorpdfstring{$C=-AMQ$}{C=-AMQ}}
 Let $Q_H$ be a critical threshold value of $Q$ given by the third condition of Theorem \ref{teoest1}. We remark that 
 when $Q>Q_H$, the positive equilibrium point $E_1$ is stable, for a fixed $\varepsilon > 0$, losing stability when $Q$ decreases, so that when $Q=Q_H$ a Hopf bifurcation occurs, recall Section \ref{sec:linear_stability}. 
 By further decreasing $Q$, we pass
from statement 2(b) ($A-M+AM>1/Q$) of Theorem \ref{teo1} to statement 2(a) ($A-M+ AM<1/Q$). This transition is due to the appearance of a new equilibrium point $E_2:=(\mathcal{U}_2,\mathcal{V}_2)$, as we detail below.

 
Since $C=-AMQ$, we have that \eqref{eq_equilibrio1} becomes
$$u\left(u^{2}+(A-M-1)u+M-A-AM+\frac{1}{Q}\right)=0,$$
        whose solutions are
$$u=0, \qquad u=\frac{1}{2}\left(1+M-A\pm\sqrt{(A+M+1)^2-4M-\frac{4}{Q}}\: \right).$$      
Let $\mathcal{U}_{1} =\frac{1+M-A + \sqrt{(A+M+1)^2-4M-\frac{4}{Q}}}{2}$ and
$\mathcal{U}_{2} =\frac{1+M-A -\sqrt{(A+M+1)^2-4M-\frac{4}{Q}}}{2}$.
\hjk{It follows from standard computations that these roots are real and satisfy 
$0< \mathcal{U}_{2} < \mathcal{U}_{1}$ if only if 
\begin{equation}
    -1 < M < 0, \quad 0 < A < 1+M, \quad \frac{4}{(A+M+1)^2-4M}<Q<\frac{1}{A+M-AM}
\end{equation}
}

\begin{mdframed}\small
    We erase this when we all agree.
    First:
    \begin{equation}
        \begin{split}
            (A+M+1)^2-4M-\frac{4}{Q}>0\\
            \underbrace{(A+M+1)^2-4M}_{>0}>\frac{4}{Q}\\
            \frac{4}{(A+M+1)^2-4M}<Q
        \end{split}
    \end{equation}
    Next:
    \begin{equation}
        \begin{split}
            1+M-A&>\sqrt{(A+M+1)^2-4M-\frac{4}{Q}} \qquad \text{(both sides positive)}\\
            (1+M-A)^2&>(A+M+1)^2-4M-\frac{4}{Q}\\
            1+M^2+A^2+2M-2A-2AM&>A^2+M^2+1+2A+2M+2AM-4M-\frac{4}{Q}\\
            -4A+4M-4AM&>-\frac{4}{Q}\\
            \frac{1}{A-M+AM}&>Q.
        \end{split}
    \end{equation}
\end{mdframed}




% With the help of Mathematica software, we compute that 
% these roots are real and satisfy 
% $0< \mathcal{U}_{2} < \mathcal{U}_{1}$ if only if 
% $$-1 < M < 0, \quad 0 < A < 1+M, \quad \frac{1}{A^2+(M-1)^2+2A(1+M)} \leq Q < \frac{1}{4(A-M+AM)}.$$
 

We are now in the position to prove the following result.
\begin{prop}
Assuming $AM+C/Q=0$, the equilibrium point $E_2=(\mathcal{U}_{2},\frac{\mathcal{U}_{2}+C}{Q})$ for system \eqref{eq_modelo1}  is a saddle point.
\end{prop}

\begin{proof} 
Replacing $u$ in $\frac{1}{Q}- J_{11}$
(see details in Appendix \ref{app:JacobianTrace})  by $\mathcal{U}_{2}$, we obtain
        \begin{equation*}
        \begin{split}
         &\frac{1}{Q}- J_{11}=3\mathcal{U}_{2}^{2}-2(M+1-A)\mathcal{U}_{2}-\left(AM+A-M-\frac{1}{Q}\right)\\
         &=-\frac{1}{2}\left(1+M-A-\sqrt{(A+M+1)^2-4M-\frac{4}{Q}}\right)\left(\sqrt{(A+M+1)^2-4M-\frac{4}{Q}}\right)<0.
         \end{split}
        \end{equation*}
        This means that $\text{det}(\mathcal{J}(E_{2}))<0$ and the eigenvalues of $\mathcal{J}(E_{2})$, given in \eqref{matriz1},
         are real with opposite signs. 
         Hence, from the above analysis, we can say that
     $E_{2}$  is a saddle point.
    \end{proof}


%It is worth noting that  when the point $P_2$ arises, then the relaxation cycle which comes from the canard explosion disappears.\hjk{This comment seems very vague at this place}

\subsection{Case \texorpdfstring{$C<-AMQ$}{C < -AMQ}}

In Section \ref{sec:linear_stability}, we showed that as $Q$ passes through its critical value $Q_H$, the positive equilibrium $E_{1}$  loses its stability and a Hopf bifurcation occurs. By further decreasing of $Q$ the equilibrium is unstable. However, numerical simulations suggest that close to the point $T_{\mathcal{C}}$, the  equilibrium gains stability  via a subcritical Hopf bifurcation.
This will be  shown in the Section \ref{TB}.
\hjk{So, this has nothing to do with another equilibrium appearing? Then it is weird that this appears in this section, no?}


In the following section we will determine the criticality of the singular Hopf bifurcation.



\hjk{Connect sections better}

==> sections/slowmanifolds.tex <==
In this section,  we follow the geometric singular perturbation technique to find the analytical expression of the locally perturbed invariant manifold ${\mathcal M}_\varepsilon^1$ as a power series in $\varepsilon$, which is used in .........

Since by Fenichel's theorem \cite{Fenichel1979}  $v=h_\varepsilon(u)$ depends smoothly on $\varepsilon$, it admits the formal power series expansion 
\begin{equation}\label{eq_seriesq}
v=h_\varepsilon(u)= h_0(u)+ \varepsilon h_1(u) + \varepsilon^2 h_2(u)+ \dots =\sum_{j=0}^{\infty}{\varepsilon^j h_j(u)}.
\end{equation}
Thus, from  the invariance property of the perturbed manifold, $v=h_\varepsilon(u)$ satisfies
 the invariance equation 
$$\dfrac{\dd v}{\dd\tau}=\dfrac{\dd h_\varepsilon(u)}{\dd u}\dfrac{\dd u}{\dd\tau}.$$

This equation may be solved explicitly for each term $h_j(u)$, 
recursively.  To carry out this procedure we
use the explicit expression for $\dfrac{\dd u}{\dd\tau}$ and $\dfrac{\dd v}{\dd\tau}$ from \eqref{slowfast1}  into the preceding equation,
then  one finds
$$
\varepsilon  h_\varepsilon(u) (u+A)(u+C + Qh_\varepsilon(u))= u(u+C) \dfrac{\dd}{\dd u}h_\varepsilon(u)\big((u+A)(1-u)(u-M)-h_\varepsilon(u) \big).
$$
Upon making the substitution of  the asymptotic expansion \eqref{eq_seriesq}, we get
\begin{equation}
\label{eq14}
\begin{split}
\varepsilon & \sum_{j=0}^{\infty}{\varepsilon^j h_j(u)} (u+A)\left(u+C- Q\sum_{j=0}^{\infty}{\varepsilon^j h_j(u)}\right)=\\
& u(u+C)\dfrac{\dd}{\dd u}\sum_{j=0}^{\infty}{\varepsilon^j h_j(u)}\left( (u+A)(1-u)(u-M)- \sum_{j=0}^{\infty}{\varepsilon^j h_j(u)}\right).
\end{split}
\end{equation}
For the calculation of the slow invariant manifold ${\mathcal M}_\varepsilon^1$,
 we assume that $u\neq 0$ and that $\frac{\dd{h}_{0}}{\dd u}(u)\neq 0$, and proceed by  gathering the common powers of $\varepsilon$ from both sides.  
 The coefficient of $\varepsilon^0$  results in
 \begin{equation}
 \label{eq_h0}
    h_{0}(u)=(u+A)(1-u)(u-M),
 \end{equation}
which is exactly the critical manifold. Similarly, the coefficients of  $\varepsilon$ from both sides of  \eqref{eq14} yield 
$$h_{1}(u)=\dfrac{h_{0}(u)(u+A)(u+C -Qh_{0}(u))}{-u(u+C){h}_{0}'(u)},$$
where ${h}_{j}' = \frac{\dd h_j}{\dd u}$.
The $\varepsilon^2$ terms in \eqref{eq14} show that
$$h_{2}(u)=\dfrac{h_{1}(u)\left((u+A)(u+C-2Qh_{2}(u))+u(u+C){h}_{1}'(u)\right)}{-u(u+C){h}_{0}'(u)}.$$
Therefore, the approximation of the perturbed invariant manifold up degree $2$ is given by
\begin{multline*}
h_\varepsilon(u)= (u+A)(1-u)(u-M)
+\varepsilon \dfrac{h_{0}(u)(u+A)(u+C -Qh_{0}(u))}{-u(u+C){h}_{0}'(u)}\\
 +\varepsilon^2 \dfrac{h_{1}(u)\left((u+A)(u+C-2Qh_{2}(u))+u(u+C){h}'_{1}(u)\right)}{-u(u+C){h}_{0}'(u)} + {\mathcal O}(\varepsilon^3).
\end{multline*}
